Semantic 3D Occupancy Mapping through Efficient High Order CRFs

Semantic 3D mapping can be used for many applications such as robot navigation and virtual interaction. In recent years, there has been great progress in semantic segmentation and geometric 3D mapping. However, it is still challenging to combine these two tasks for accurate and large-scale semantic mapping from images. In the paper, we propose an incremental and (near) real-time semantic mapping system. A 3D scrolling occupancy grid map is built to represent the world, which is memory and computationally efficient and bounded for large scale environments. We utilize the CNN segmentation as prior prediction and further optimize 3D grid labels through a novel CRF model. Superpixels are utilized to enforce smoothness and form robust P N high order potential. An efficient mean field inference is developed for the graph optimization. We evaluate our system on the KITTI dataset and improve the segmentation accuracy by 10% over existing systems.

==> dense_crf.tex <==
Our fully connected 3D CRF model is based on a 2D dense CRF in \cite{krahenbuhl2012efficient}, which is a filter-based method for performing fast approximate maximum posterior marginal (MPM) inference in multi-label CRF models with fully connected pairwise terms and Gaussian edge potentials. We use the same filter-based update technique, while using the 3D features.

\subsubsection{Notation Definition}
Consider a random field X defined over a set of variables $\{X_1, ..., X_N\}$ conditioned on an 3D reconstruction map $\textbf{M}$. We assume there is a random variable associated with each 3D grid in the 3D reconstruction map $\mathcal{N} = \{ 1,...,N\}$ and the random variable takes value from a label set $\mathcal{L} = \{l_1, ..., l_L\}$. Then we have the posterior:
\begin{equation}
   \label{eq:dense-crf-p}
    P(\textbf{X}|\textbf{M}) = \frac{1}{Z(\textbf{M})} exp(-E(\textbf{X}|\textbf{M}))
\end{equation}

A conditional random field (\textbf{M}, \textbf{X}) is characterized by a Gibbs distribution:
\begin{equation}
   \label{eq:gibbs}
    P(\textbf{X}|\textbf{M}) = \frac{1}{Z(\textbf{M})} exp(-\sum_{c\in \mathcal{C_G}}\phi_c(\textbf{X}_c|\textbf{M}))
\end{equation}
where $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ is a graph on $\textbf{X}$ and each clique $c$ in a set of cliques $\mathcal{C_G}$ induces a potential $\phi_c$. The Gibbs energy of a labeling $x \in \mathcal{L}^N$ is $E(x|\textbf{M}) = \sum_{x\in \mathcal{C_G}} \psi_c(x_c)$, where we use $\psi_c(x_c)$ to denote $\phi_c(x_c|\textbf{M})$ for simplicity.

\subsubsection{3D Dense CRF Description}
With the notation definition above, we can describe our 3D dense CRF. In 3D dense CRF, we have each single node and connected node pairs as cliques in Eq \ref{eq:gibbs}. Thus, we can express the 3D fully connected pairwise CRF with unary and pairwise cliques in Gibbs energy as: 

\begin{equation}
   \label{eq:dense-crf-e}
    E(\textbf{X}|\textbf{M}) = \sum_{i \in \mathcal{N}}\psi_u(x_i) + \sum_{i<j \in \mathcal{N}} \psi_p(x_i, x_j)
\end{equation}

% label distribution => unary
%% TODO !!!!  ------ describe in detail in later section about what is used as unary potential.
The unary potential $\psi_u(x_i)$ is a label distribution for each 3D grid. It is an average of the label distribution of the corresponding pixels in video images. The label distributions of pixels are computed independently for each pixel by an image classifier. The image classifier produces a distribution over the label assignment $x_i$ given image features. One can use any image classifier to acquire the label distribution. Figure \ref{fig:unary exm} shows the labeling produced by the unary classifiers and labels mapped the 3D. Note that the unary labeling is generally noisy and inconsistent.

\begin{figure}
    \centering
    \subfigure[] {
    \includegraphics[scale=0.10]{separate_3d_crf/unary_classifier.jpg}
    }
    \subfigure[] {
    \includegraphics[scale=0.25]{separate_3d_crf/unary_3d_grid.png}
    }
    \caption{(a) Unary classifier in 2D image. (b) Unary classfier projeccted into 3D grid space. Each grid contains a probability distribution projectted from 2D image. Different color represents the different labels.
    } 
    \label{fig:unary exm}
\end{figure}

The pairwise potentials in our model have the form:
\begin{equation}
   \label{eq:pairwise-potential}
    \psi_p(x_i, x_j) = \mu (x_i, x_j) \sum_{m=1}^K w^{(m)}k^{(m)}(\textbf{f}_i, \textbf{f}_j)
\end{equation}

where each $k^{(m)}$ is a Gaussian kernel
\begin{equation}
   \label{eq:dense-crf-e}
    k^{(m)}(\textbf{f}_i, \textbf{f}_j) = exp(-\frac{1}{2}(\textbf{f}_i - \textbf{f}_j)^T \Lambda^{(m)} (\textbf{f}_i - \textbf{f}_j))
\end{equation}
 
For multi-class 3D semantic labeling, we are currently using a two kernel potentials defined based on the color vector mapped to the 3D grid $I_i$ and $I_j$ and also the position of the 3D grid $p_i$ and $p_j$:
 
 \begin{equation}
   \label{eq:kernel}
   \begin{split}
    k(\textbf{f}_i, \textbf{f}_j) = &w^{(1)}exp\Big( -\frac{|p_i -p_j| }{2\theta_\alpha^2} - \frac{|I_i - I_j |}{2 \theta_\beta^2} \Big)  \\
    &+ w^{(2)} exp\Big(  -\frac{|p_i -p_j| }{2\theta_\gamma^2}  \Big) 
    \end{split}
\end{equation}

%  do we learn u(x_i, x_j) instead of using the potts model ????? no
We use the simple Potts model for the compatibility function $\mu$ with $\mu(x_i, x_j) = [x_i \neq x_j]$, which introduces a penalty for nearby similar pixels that are assigned different labels.
 
 
 \subsubsection{Filter-based Efficient Inference for 3D Dense CRF}
According to \cite{krahenbuhl2012efficient}, we derive a very efficient inference algorithm for 3D dense CRF based on a mean field approximation to the CRF distribution and high-dimensional filtering.
 
 Instead of exactly deriving the distribution $P(X)$, we use mean field to approximate $P(X)$ with a distribution $Q(X)$ that minimize the KL-divergence $D(Q||P)$ among all distributions $Q$ that having the form $Q(X) = \prod_i Q_i(X_i)$.
 
 Based on \cite{koller2009probabilistic}, we know that the iterative update equation for each $Q_i(X_i)$ is:
  \begin{equation}
   \label{eq:mf-update}
   \begin{split}
    Q_i(x_i = l) = &\frac{1}{Z_i}exp \Big\{ -\psi_u (x_i) - \sum_{l' \in \mathcal{L}}\mu(l,l') \\
    &  \sum_{m=1}^K w^{(m)}   \sum_{j \neq i} k^{(m)} (\textbf{f}_i, \textbf{f}_j) Q_j(l') \Big\}
    \end{split}
\end{equation}

We can use a message algorithm as \cite{krahenbuhl2012efficient} with the messages
  \begin{equation}
   \label{eq:msg}
   \begin{split}
    \tilde{Q}_i^{(m)}(l) \gets \sum_{j \neq i} k^{(m)} (\textbf{f}_i, \textbf{f}_j) Q_j(l)%\sum_{j \in \mathcal{V}}
    \end{split}
\end{equation}

Since we have Gaussian potentials, the message passing step can also be expressed as a convolution with a Gaussian kernel $G_{\Lambda^{(m)}}$ in feature space:
  \begin{equation}
   \label{eq:conv}
   \begin{split}
    \tilde{Q}_i^{(m)}(l) & = \sum_{j \in \mathcal{V}}  k^{(m)} (\textbf{f}_i, \textbf{f}_j) Q_j(l) - Q_j(l) \\
    & = [G_{\Lambda^{(m)}}\otimes Q(l)](\textbf{f}_i) - Q_i(l)
    \end{split}
\end{equation}

In a d-dimensional feature space, the naive message passing algorithm is $O(N^dL^2)$. However, since d-dimensional Gaussian filtering can be done with d times 1-dimensional Gaussian filtering for each dimension, the complexity can be reduced to $O(dNL)$, where d is the number of features, N is the number of 3D grids and L is the number of labels.
 
 
 
 
 
 
 
 
 

==> high_order.tex <==
While the dense CRF generates constraint among every two pixels, it lacks the ability to express more complicated and meaningful constraints, such as enforcing the label consistency over homogeneous regions; objects should be above the ground pixels, etc.
Thus, we include high-order potentials $\psi_s$ in the CRF model of Equation \ref{eq:pariwise_def}, which has been shown to provide important priors for segmentation \cite{ladicky2010graph}. While the orgirinal P$^n$ Potts Model rigidly enforces the label consistency, Kohli proposed a Robust Potts Model whose cost is enforced by the two high order potentials changes with the number of variables in the clique not taking the dominant label \cite{kohli2009robust}. However, this robustness is achieved at the cost of the time complexity. While the $P^n$ Potts Model only required linear time to the clique size, the time complexity for Robust $P^n$ Potts Model is exponential to the clique size. 

Instead, we propose our own high order potential in this paper, which preserves both efficient computation time and non-rigid label consistency enforcement. As shown in \cite{geiger2012we}, the high order $P^n$ potentials are equivalent to the minimization of a pairwise graph defined over the same clique $X_c$ and a single auxiliary variable $y_c$. For example, the five nodes added in the right image of Figure \ref{fig:auxilliary} are the five superpixels represented by an auxiliary node. They are connected to the pixels that are inside the superpixel. Thus in our high order potential, we use the auxiliary node to represent the superpixel. We acquire the label distribution for each clique and our cost is enforced by two high order potentials changes with the label consistency of some particular label distribution. 

\begin{figure}[h]
  \centering     %%% not \center
       \includegraphics[scale=0.08]{separate_3d_crf/auxilliary.jpg}   
   \caption{Representing superpixel as an auxiliary node  \cite{russell2009associative}}     \label{fig:auxilliary}
\end{figure}

More specifically, in our high order potential, we first represent each clique using the average position and average color in this clique. We then obtain the clique label distribution by doing a dense CRF on the superpixel level. After acquiring the superpixel label distribution, we define our high order potential as:
 
\begin{equation}
   \label{eq:superpixel_cliques}
\psi^{sp}_c(\mathbf{x}_c) = 
\begin{cases}
	-\gamma_l s_{cl}      & \quad \text{if } \forall i \in c \text{,} x_i = l\\
        -\gamma_{min}  & \quad \text{Otherwise}\\
\end{cases}
\end{equation}

where $s_{cl}$ is the label distribution of the superpixel auxiliary node. So this potential gives cost  $\gamma_l  s_{cl}$ if all the pixels in the segment all take the label $l$. It encourages all the pixels inside one superpixel having the same label that has high probability in superpixel label distribution. Each pixel not taking the label $l$ is encouraged less with cost $-\gamma_{min}$. 

Similar to 3D dense CRF, we can derive the update function for high order CRF:

\begin{equation}
   \label{eq:high-order-update}
   \begin{split}   
	&\sum_{\{ \textbf{x}_c | x_i = l\}} Q_{c-i}(\textbf{x}_{c-i}) \dot \psi_c^{potts}(\textbf{x}_c) \\
	=& - \bigg ( \prod_{j \in c, j \neq i} Q_j (x_j = l) \bigg) \gamma_l s_{cl} \\
	&- \bigg ( 1 - \bigg(\prod_{j \in c, j \neq i} Q_j (x_j = l) \bigg) \bigg)\gamma_{min}
  \end{split}   
\end{equation}

which contribute $O(L max_c (|c|) |C|)$ to each parallel update. Here, $|c|$ is the size of a superpixel and $|C|$ is the number of superpixels. If we assume each pixel can belong to at most $M$ cliques, we can reexpress this as $O(MNL)$. Thus, in our high order potential setting, we achieve the time complexity linear to the number of 3D grid N, which effectively preserves the $O(dNL^2)$ complexity of the dense pairwise updates (assuming $M \approx d$).

==> overview.tex <==
The whole system diagram is shown in Fig \ref{fig:kitti crf whole system}. The input to our system is a series of stereo pair images and the output is an incrementally built 3D semantic grid map. We divided the problem into two parts: geometric 3D reconstruction and semantic 3D labelling through CRF optimization. Scrolling occupancy grid map is built from the SLAM to represent the world and each occupied grid is a node in the 3D CRF. We then use 2D CNN network to predict per-pixel label distribution and transfer them to 3D, treated as the CRF unary distribution. 2D superpixel is also transferred to 3D grids to build a hierarchical CRF.


\begin{figure*}
    \centering
    \includegraphics[scale=0.55]{whole_system2.PNG}
    \caption{Overview of our system. (a) Input stereo image pairs. (b) Geometric 3D reconstruction using ORB SLAM \cite{mur2015orb}   and occupancy mapping \cite{scherer2012river}\cite{fang2016robust}. (c) 2D semantic segmentation using CNN \cite{yu2015multi}, treated as CRF unary. (d) Superpixel clique generation using SLIC \cite{achanta2012slic} to enforcement consistency within a region. (e) Hierarchical CRF model. We develop efficient mean field inference for hierarchical CRF in 3D grid space. (f) Final semantic mapping after 3D CRF optimization.
} 
    \label{fig:kitti crf whole system}
\end{figure*}


%stereo image pairs are used to produce three major components 1) \textbf{Color 3D cloud}: given stereo image pairs, we generate depth and estimate six DoF camera pose using SLAM algorithm. Next, we fuse the depth into a global 3D grid map. 2) \textbf{Unary label distribution}: We use random forest to compute unary label distribution for each pixel in 2D images and project it into 3D grid map. 3) \textbf{Superpixel Clique}: We also use SLIC algorithm to generate superpixels from images treated ad CRF cliques. After acquiring the three major components, we project both pixel features and superpixel features into 3D space. With the defined 3D unary and cliques, our proposed high order CRF model is utilized to optimize the final distribution in 3D grid space.

